Optimal Stopping with Multi-Dimensional Comparative Loss Aversion

Despite having the same basic prophet inequality setup and model of loss aversion, conclusions in our multi-dimensional model differs considerably from the one-dimensional model of Kleinberg et al. For example, Kleinberg et al. gives a tight closed-form on the competitive ratio that an online decision-maker can achieve as a function of $\lambda$, for any $\lambda \geq 0$. In our multi-dimensional model, there is a sharp phase transition: if $k$ denotes the number of dimensions, then when $\lambda \cdot (k-1) \geq 1$, no non-trivial competitive ratio is possible. On the other hand, when $\lambda \cdot (k-1) < 1$, we give a tight bound on the achievable competitive ratio (similar to Kleinberg et al.). As another example, Kleinberg et al. uncovers an exponential improvement in their competitive ratio for the random-order vs. worst-case prophet inequality problem. In our model with $k\geq 2$ dimensions, the gap is at most a constant-factor. We uncover several additional key differences in the multi- and single-dimensional models.

==> sections/properties.tex <==
\section{The Suffering Prophet}
\lindanote{TODO: shorten this section. }

\lindanote{TODO: new intro}

\label{properties}
In this section we will highlight some additional properties that are specific to our model, with a focus on the biased prophet. We will show that:
\begin{enumerate}
    \item 
    In our model, the biased prophet could be infinitely worse off than the biased agent. In contrast, in \cite{kleinberg2021optimal}'s model (without multiple dimensions), the biased prophet always obtains at least as much utility as that of online agents. 
    \item 
    An agent suffering from comparative loss aversion can be better off with a distinctly worse set of candidates. 
\end{enumerate}
Our examples illustrating these properties is similar in spirit to the example in Section~\ref{example}. 


 
We will start our analysis by considering some prophet inequalities. Prior to exploring these however, we need to establish a distinction between a "biased prophet" and an "unbiased prophet."   
In the one dimensional case(i.e. that explored in \citet{kleinberg2021optimal}), the distinction is unnecessary. Since the prophet selects the maximum valued candidate and receives utility equal to their value, there is no loss aversion factor to subtract. However, in multiple dimensions, even the maximum valued candidate could still have lower values than other candidates on certain dimensions. Thus, the utilities of a biased prophet and unbiased prophet can be dramatically different. 

Furthermore, in the one dimensional case, the utility of the prophet is always an upper bound on the utility of the biased gambler, however in the multi-dimensional case, this is no longer true.  To explore this phenomenon, there are two prophet inequalities which are of particular interest: (1) the ratio of the value of the candidate the biased gambler selects to the value of the candidate that the biased prophet selects, (2) the ratio of the utility received by the biased gambler to the utility received by the biased prophet. We now show that there exist adversarial sequences such that the utility received by a biased prophet is a lower bound on the utility received by a biased gambler for all possible strategies, yet the values of their chosen candidates are equivalent.
\begin{theorem}
\label{ProphetParadox}
 Let r denote the position of the candidate selected by the biased prophet and t denote the position of the candidate selected by the biased gambler on a sequence $\sigma$. There exists $\sigma$ such that for all $r, t \in \{1...n \}$,  $\sigma^{(t)} = \sigma^{(r)}$ and $U_{g_b}(\sigma, t) \geq U_{p_b}(\sigma, r)$.  
\end{theorem}
\begin{proof}
Consider an adversarial sequence $\sigma$ of length k, such that there are k candidates each of which has a k-dimensional value vector. Moreover, let q be some fixed constant such that $q > 1$, and let the value vector of the $i^{th}$ candidate be q at index i and 0 everywhere else. Semantically, the rational value of all candidates in $\sigma$ is q, i.e. for all $i, j \in \{1...n \}, \| \sigma^{(i)} \|_1 = \| \sigma^{(j)} \|_1 = q$. Our sequence appears as follows:
\begin{align*}
   (q, 0 , ..., 0, 0),(0, q , ..., 0, 0), \cdots , (0, 0 , ..., q, 0), (0, 0 , ..., 0, q). 
\end{align*}

Trivially, since the prophet sees all candidates, it follows that the "super candidate" imagined by the biased prophet is $s^{(k)}=(q, q,…, q) \in \mathbb{R}^k$. Since all candidates have rational value q, it follows that the biased prophet receives the same utility regardless of which candidate, r,  they select. Specifically, we have:
\begin{align*}
    U_{p_b}(\sigma) = \| \sigma^{(r)} \|_1 - \lambda \bigg(\| s^{(k)} \|_1 - \|\sigma^{(r)} \|_1\bigg) =  q\bigg(1 -  \lambda (k - 1)\bigg).
\end{align*}

Observe that, in contrast, the gambler who selects candidate t sees only t candidates total and thus their super candidate has a value vector with q's in the first t indices and zeros thereafter. Thus, he gambler receives the following utility: 
\begin{align*}
    U_{g_b}(\sigma, t) = \| \sigma^{(t)}\|_1 - \lambda \bigg(\| s^{(t)}\|_1 - \| \sigma^{(t)} \|_1\bigg) = q\bigg(1 - \lambda (t - 1)\bigg).
\end{align*}

Since $t \in [k]$, for $k \geq 2$, $q > 1$ and $\lambda > 0$, we have: 
$
    q\bigg(1 - \lambda (k - 1)\bigg) \leq q \bigg(1 - \lambda (t - 1) \bigg)$, which in turn implies the claim, namely that $\forall t \in \{1...|\sigma| \}, U_{g_b}(\sigma, t) \geq U_{p_b}(\sigma, r).$

\end{proof}
For this sequence, the fewer candidates a biased agent sees, the better off they are. The gambler can stop early and see fewer, whereas, in contrast, a biased prophet cannot escape seeing all candidates, and thus receives lower utility than the gambler. In fact the payoff of a biased prophet can be arbitrarily negative for adversarial sequences whereas the gambler is always guaranteed one strategy that yields positive payoff, namely selecting the first candidate. Under our adversarial sequence, regardless of which candidate the prophet chooses they just receive payoff of $q(1 - \lambda(k-1))$, and as $\lambda$ or k increase, this payoff becomes increasingly negative.   

Whereas in one dimension, a biased prophet guaranteed to always outperform both a biased and unbiased gambler, in multiple dimensions, there is no such guarantee. Comparative loss aversion leads to a fundamental breakdown in the traditional semantics of prophet inequalities, such that in the multi-dimensional setting the prophet's clairvoyance is a curse. 
\subsection{The Paradox of Quality}
In this section, we explore a phenomenon in which an agent suffering from comparative loss aversion can be better off with a distinctly worse set of candidates. We will more formally define what we mean by this and give example instances for which this occurs.

\begin{definition}[Point-wise Dominance]
Sequence $\sigma'$ point-wise dominates sequence $\sigma$ if for all $i$, $\| \sigma'^{(i)} \|_1 \geq \| \sigma^{(i)} \|_1$.
\end{definition} 
\begin{claim}
There exist $\sigma$ and $\sigma'$, such that  $\sigma'$ point-wise dominates $\sigma$, yet both prophet and gambler are better off playing optimally on $\sigma$ than $\sigma'$.
\end{claim}
\begin{proof}
Let $\beta = \lambda \cdot (k-1)$, and let $ \beta > \epsilon > 0$, where $\epsilon$ is a small positive constant. Consider the following sequence $\sigma$:   
\begin{align*}
    &(1, 0, \cdots, 0), (1, 0, \cdots, 0), \cdots, (1, 0, \cdots, 0), (1 + \epsilon, \cdots, 0, 0).
\end{align*}
Similarly, consider the following $\sigma'$
\begin{align*}
    &(1, 0, \cdots, 0), (0, 1, 0, \cdots, 0), \cdots, (0, \cdots, 0, 1), (1 + \beta, 0, \cdots, 0).
\end{align*}
Observe that $\sigma'$ point-wise dominates $\sigma$. Moreover, observe that on $\sigma$ the best the gambler can do is to select the final candidate, i.e. $\argmax \limits_t (U_{g_b}(\sigma, t)) = n$, where n is the final option in the sequence $\sigma$. This yields the following utility: 
$$U_{g_b}(\sigma, n) =\|(1 + \epsilon, \cdots, 0, 0) \|_1 =  1 + \epsilon.$$ 
Observe that since all vectors were only non-zero along the first dimension and the selected option had the highest value on this dimension, there was no loss aversion factor to subtract. Now let's consider $\sigma'$. On $\sigma'$, the optimal strategy for the gambler is to select either the first or the last option, i.e. $\argmax \limits_t (U_{g_b}(\sigma', t)) = \{1, n\}$. For t= 1, the calculations are simple, yielding $U_{g_b}(\sigma', 1) = \| (1, 0, \cdots, 0)\|_1 = 1$. For $t=n$, they are slightly more involved:
\begin{align*}
     U_{g_b}(\sigma', n) &= \| (1 + \beta, 0, \cdots, 0) \|_1 - \lambda \bigg( \|(1 + \beta, 1, \cdots, 1) \|_1 - \| (1 + \beta, 0, \cdots, 0) \|_1\bigg)\\
    &= (1 + \beta) - \lambda \bigg( ((1 + \beta) + (k-1)) - (1 + \beta) \bigg)= (1 + \beta) - \lambda(k-1) \\
    &= 1 + \lambda(k-1) - \lambda(k-1) = 1. 
\end{align*}
Note that last step is just substituting in the definition of $\beta$.
The gambler is better off playing optimally on $\sigma$ than on $\sigma'$. For the prophet, they just select the maximum valued option for both $\sigma$ and $\sigma'$. Namely, they select the last option in both cases, yielding utility $U_{p_b}(\sigma, n) = 1 + \epsilon$ and $U_{p_b}(\sigma', n) = 1$. Thus, the prophet is also better off playing optimally on $\sigma$ than on $\sigma'$.
\end{proof}
We now consider a more extreme scenario in which all candidates are distinctly better in $\sigma'$ than in $\sigma$. Let's formally define what we mean by that:
\begin{definition}[Higher Quality]
If sequences $\sigma$ and $\sigma'$ are such that the minimum valued option in $\sigma'$ is of greater rational value than the maximum valued option in $\sigma$, then we say that $\sigma'$ is of higher quality than $\sigma$. More formally $\sigma'$ is of higher quality than $\sigma$ if and only if:
$$ \min\limits_{w : w \in \{1...n'\}} \|\sigma'^{(w)}\|_1 > \max\limits_{u : u \in \{1...n\}} \|\sigma^{(u)} \|_1$$
\end{definition}

\begin{claim}
\label{claim:prophetquality} 
There exist $\sigma$ and $\sigma'$, where $\sigma'$ is of higher quality than $\sigma$,  such that for all $t \in \{ 1... n \}$ and all $r \in \{1... n' \}$, $U_{p_b}(\sigma, t) > U_{p_b}(\sigma', r)$. Informally, even if a sequence $\sigma'$ is of higher quality than another sequence $\sigma$, the prophet is not is not necessarily better off playing optimally on $\sigma'$ than on $\sigma$.
\end{claim}
\begin{proof}
Let us simply re-use the example sequence from theorem \ref{ProphetParadox} with different settings of q. Recall that in this sequence, all candidates have the same rational value, namely q. To construct $\sigma$ simply set $q$ such that $q > 1$. To construct $\sigma'$, simply set $q' = qk$, where k is the number of dimensions in the value vectors of candidates.  Moreover, recall the utilities we derived for the biased prophet in theorem \ref{ProphetParadox}. We re-use them here substituting in q' where appropriate:
$$U_{p_b}(\sigma, t) =  q(1 -  \lambda (k - 1)) $$ 
$$U_{p_b}(\sigma', r) =  q'(1 - \lambda (k - 1)) = qk(1 - \lambda (k - 1)) $$
If $ k > 1$ and $\lambda > \frac{1}{k-1}$, then $q(1 -  \lambda (k - 1)) > qk(1 - \lambda (k - 1))$ thus proving the claim. 
\end{proof}
\begin{corollary}
If $k > 1$ and $\lambda > \frac{1}{k-1}$, then for the sequence in the previous claim, as q grows larger the prophet's utility gets lower.
\end{corollary}
Note that since all candidates have rational value q, this is equivalent to saying that even as we improve the quality of all individual candidates, we make the prophet worse off. Now let's consider the case of the gambler. 
\begin{claim}
\label{claim:gamblerquality} 
There do not exist sequences $\sigma$ and $\sigma'$ such that $\sigma'$ is of higher quality than $\sigma$ and for all t and r, $U_g(\sigma, t) > U_g(\sigma', r)$. Informally, if a sequence $\sigma'$ is of higher quality than another sequence $\sigma$, then the gambler is always better off playing optimally on $\sigma'$ than on $\sigma$. 
\end{claim}
\begin{proof}
By the definition of higher quality, the maximum value in $\sigma$ is less than the minimum value in $\sigma'$. Let the gambler simply select the first option in $\sigma'$. They are guaranteed to get utility greater than or equal to the value of the minimum valued option in $\sigma'$. Since this is greater than the value of the maximum valued option in $\sigma$, it follows that for all t and r, $U_g(\sigma, t) < U_g(\sigma', r)$. 
\end{proof}
\begin{theorem}[The Prophet Paradox, Part II]
If sequence $\sigma'$ is of higher quality than sequence $\sigma$, it must be the case that a biased gambler playing optimally is better off playing on $\sigma'$, however a biased prophet playing optimally can be worse off for adversarial sequences. 
\end{theorem}
\begin{proof}
The theorem follows directly from claims \ref{claim:prophetquality} and \ref{claim:gamblerquality}.
\end{proof}
Once again, the gambler can be better off than the prophet. For our example sequence, as the values of the candidates improve, the biased prophet becomes increasingly unhappy with whatever candidate they end up choosing. In essence, as the objective quality of their options increases, the subjective quality of their options decreases due to comparative loss aversion. 




==> sections/removed_content.tex <==
\section{Behavioral Analysis}
Intuitively, information about additional candidates makes our agent less satisfied with their ultimate decision. Moreover, this effects the prophet worse than the gambler; since the gambler will never know the candidates that would come after the one they pick, they can't feel loss over having turned them down. In the case of our biased agent, ignorance truly is bliss. In behavioral literature\cite{schwartz2004paradox}, the phenomenon in which knowledge of additional candidates decreases happiness with one's chosen candidate is referred to as "The Paradox of Choice". We borrow the behavioral terminology here and use it explore additional aspects of the paradox of choice that occur in our model but not in the original model of \citet{kleinberg2021optimal}.
\begin{definition}[Paradox of Choice] If adding a candidate makes the utility of an agent decrease, we refer to this as a paradox of choice. 
\end{definition}
Note that paradoxes of choice cannot occur for fully rational agents since they will simply disregard additional candidates that do not improve the maximum. Notably, \citet{kleinberg2021optimal} already showed a paradox of choice for the one dimensional case. In particular, in their monotonicity results, they showed that adding candidates to the beginning of a sequence can harm the utility of a biased gambler. 

Observe that in the example used in theorem \ref{ProphetParadox}, as the number of candidates seen increases, the utility received by the agent decreases. Moreover, observe that, by construction of the example, the order in which the candidates are presented has no effect on the analysis. All items have the same rational utility, yet as the number of items seen increases, the biased utility decreases linearly. This is an extreme example of the paradox of choice at work. 
\subsection{Applying The Model}
We can extend the intuition from theorem \ref{ProphetParadox} to create models which appear more behaviorally realistic than the contrived example used in the proof of the theorem, yet which still yield paradoxes of quality and choice. In particular, consider the scenario in which all candidates have the same values for all features except for one salient feature per candidate. There is empirical evidence \cite{higgins1996activation} suggesting that people reduce phenomena to salient features and can only perceive differences between stimuli if their magnitude exceeds certain thresholds.  We consider a scenario in which most features across candidates are assigned the same value, and all noticeably better features are assigned another greater value. In particular, we start with the case where each candidate is advantaged along a different dimension. 
\newline 
\newline 
\textbf{Differently Advantaged Candidates}
As in theorem \ref{ProphetParadox}, consider an adversarial sequence $\sigma$ in which there are k candidates, each of which has values along k distinct dimensions. Let "a" be the standard value assigned to a non-salient features, i.e. features which are perceived as being normal/unexceptional, and let $a > 0$. Moreover, let q be some fixed constant such that $q> 1$. Let the value vector of the i-th candidate be $a +q $ at index i and a everywhere else. Trivially, since the prophet sees all candidates, it follows that the "super candidate" seen by the biased prophet is $s^{(k)}= [a+q, a+q,…,a+q] \in R^k$. 
\begin{align*}
    & v^{(1)} = [a+q, a , ..., a, a]\\
    & v^{(2)} = [a, a+q , ..., a, a]\\
    &\qquad \cdots \\
    & v^{(k-1)} = [a, a , ..., a+q, a]\\
    & v^{(k)}   = [a, a , ..., a, a+q]\\
\end{align*}
Since all the value vectors for the candidate set are $a+q$ at only one index, it follows that the biased prophet(i.e. an online decision maker) receives the same utility $U_p(\sigma, t)$ regardless of selected candidate r. We have:
$$U_p(\sigma, r) = \| v^{(r)} \|_1 - \lambda \bigg(\| s^{(k)}\|_1 - \|v^{(r)} \|_1\bigg) = (ak + q) - \lambda \bigg( (a+q)k - (ak + q)\bigg) = ak + q\bigg(1 -  \lambda (k - 1)\bigg)$$
Similarly for the gambler who stops at candidate r in the sequence, we have: 
$$U_g(\sigma, r) = \| v^{(r)} \|_1 - \lambda \bigg(\| s^{(r)}\|_1 - \|v^{(r)} \|_1\bigg) = (ar + q) - \lambda \bigg( (a+q)r - (ar + q)\bigg) = ar + q\bigg(1 -  \lambda (r - 1)\bigg)$$
Observe that the prophet's utility is negative when $\lambda > \frac{1}{k-1}$ and $q \geq \frac{ak}{( \lambda(k-1) - 1 )}$, and as q grows beyond this point, the prophet's utility grows increasingly negative. Similarly, the gambler's utility is negative when r is greater than 1, $\lambda > \frac{1}{r-1}$, and $q \geq \frac{ar}{( \lambda(r-1) - 1 )}$. As q grows beyond this point, the prophet's utility grows increasingly negative. Thus, the paradoxes of quality and choice occur for this example as well. At an intuitive level, it appears that the paradoxes occur when candidates are advantaged along different dimensions but nevertheless are otherwise of similar overall quality. 

